Power-up! What Can Generative Models Do for Human Computation Workflows?

We are amidst an explosion of artificial intelligence research, particularly around large language models (LLMs). These models have a range of applications across domains like medicine, finance, commonsense knowledge graphs, and crowdsourcing. Investigation into LLMs as part of crowdsourcing workflows remains an under-explored space. The crowdsourcing research community has produced a body of work investigating workflows and methods for managing complex tasks using hybrid human-AI methods. Within crowdsourcing, the role of LLMs can be envisioned as akin to a cog in a larger wheel of workflows. From an empirical standpoint, little is currently understood about how LLMs can improve the effectiveness of crowdsourcing workflows and how such workflows can be evaluated. In this work, we present a vision for exploring this gap from the perspectives of various stakeholders involved in the crowdsourcing paradigm -- the task requesters, crowd workers, platforms, and end-users. We identify junctures in typical crowdsourcing workflows at which the introduction of LLMs can play a beneficial role and propose means to augment existing design patterns for crowd work.

==> sections/sec-background.tex <==
\section{Background}

The research field of human computation has dedicated many efforts to the investigations of LLMs as work assistants and towards crowdsourcing workflows. We briefly provide a background on LLMs as work assistants and crowdsourcing workflows, highlighting those works where the two intersect.

% \subsection{Large Language Models Supporting Human Computation}
\subsection{Large Language Models as Work Assistants}
% Large language models (LLMs) have shown promising natural language generation capability and have been proven to be of great potential in supporting human for daily  work~\cite{bommasani2021opportunities}.
We are in the midst of an explosive growth in popularity for ChatGPT~\cite{openai2022chatgpt}, which indicates a promising future of using LLMs as work assistants. Due to such powerful generative capability, more and more researchers have started to introduce generative LLMs as work assistants. 
For example, powerful generative LLMs have shown human-comparable writing skills in story generation~\cite{yuan2022wordcraft}, scientific writing~\cite{gero2022sparks}, etc. Meanwhile, LLMs also showed promising assistance capability in complex tasks like coding~\cite{friedman_2021}, drug discovery~\cite{liu2021ai}, and question generation for education needs~\cite{wang2022towards}.

% Corwdsourcing has been widely adopted in machine learning practice to obtain high-quality annotations with human intelligence.
Crowdsourcing has been widely adopted in machine learning practice to obtain high-quality annotations with human intelligence. Attracted by the promising future of LLMs in work assistance, researchers started to apply LLMs in assisting crowd workers~\cite{liu2022wanli,bartolo2021models}. On the one hand, LLMs can generate high-quality candidates for annotation, which reduced the working load for crowd workers. On the other hand, LLMs can also generate natural language explanations~\cite{wiegreffe2022reframing} for annotations, which further contribute to the trustworthiness and explainability of such human-AI collaboration.

% \begin{itemize}
%     \item collaborative writing
%     \item dataset annotation, curation
%     \item others: education needs (question generation), program synthesis
% \end{itemize}

\subsection{Crowdsourcing Workflows}

Crowdsourcing is a paradigm in which researchers or other stakeholders request the participation of the crowd, who contribute their knowledge, expertise, and experience~\cite{estelles2012towards}. \textit{Workers} within the crowd are asked to solve large-scale problems. Oftentimes, these problems are broken down into smaller, single units of work, i.e., \textit{tasks}. Tasks can range in purpose including labelling images, editing text, or finding information on specific topics~\cite{gadiraju2014taxonomy}. \textit{Crowdsourcing workflows} are distinct patterns that manage how large-scale problems are decomposed into tasks to be completed by workers. The crowd-powered word processor Soylent applies the \textit{Find-Fix-Verify} workflow to produce high-quality text by separating tasks into generating and reviewing text tasks~\cite{bernstein2010soylent}. The \textit{Iterate-and-Vote} workflow has been deployed in creating image descriptions, where workers are asked to write descriptions of images to assist those who are blind~\cite{little2010exploring}. Subsequent voting tasks are used to decide on the optimal description.~\citet{chen2015crowdmr} introduce CrowdMR, which combines the \textit{Map-Reduce} workflow with crowdsourcing to facilitate the solving of problems that require both human and machine intelligence, i.e.,``AI-Hard" problems~\cite{yampolskiy2012ai}. 

More complex problems, such as software engineering or system design problems, require more complex workflows.~\citet{retelny2017no} investigate the relationship between the need for adaptation and complex workflows within crowdsourcing, finding that the current state of crowdsourcing workflows are inadequate for providing the necessary adaptation that complex workflows require. \ujcomment{Consider writing a couple of lines about these -- \cite{}} With the rise of the GPT family, Bart~\cite{lewis2019bart}, and other LLMs, we argue the need to investigate whether such LLMs provide a tool to reimagine crowdsourcing workflows, complex or otherwise.
